A Pragmatic Approach for Measuring Maintainability of DPRA Models

Dynamic Probabilistic Risk Assessment (DPRA) is a powerful concept that is used to evaluate design and safety of complex industrial systems. A DPRA model uses a conceptual system representation as a formal basis for simulation and analysis. In this paper we consider an adaptive maintenance of DPRA models that consist in modifying and extending a simplified model to a real-size DPRA model. We propose an approach for quantitative maintainability assessment of DPRA models created with an industrial modeling tool called PyCATSHOO. We review and adopt some metrics from conceptual modeling, software engineering and OO design for assessing maintainability of PyCATSHOO models. On the example of well-known "Heated Room" test case, we illustrate how the selected metrics can serve as early indicators of model modifiability and complexity. These indicators would allow experts to make better decisions early in the DPRA model development life cycle.

==> Sections/listings.tex <==

%%%%%%%%%%%%
%======== Listing for Python
\usepackage{listings}
\usepackage{textcomp}
\usepackage{color}
\usepackage{tikz}
\usetikzlibrary{arrows,automata}
%=========lstset==============
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
 
\lstset{style=mystyle}
%========================
%\usepackage[utf8]{inputenc}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{8} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{8}  % for normal
%=========python==========
% Python style for highlighting
\newcommand\pythonstyle{\lstset{
language=Python,
basicstyle=\ttm,
otherkeywords={self},             % Add keywords here
keywordstyle=\ttb\color{deepblue},
emph={MyClass,__init__},          % Custom highlighting
emphstyle=\ttb\color{deepred},    % Custom highlighting style
stringstyle=\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false            % 
}}


% Python environment
\lstnewenvironment{python}[1][]
{
\pythonstyle
\lstset{#1}
}
{}

% Python for external files
\newcommand\pythonexternal[2][]{{
\pythonstyle
\lstinputlisting[#1]{#2}}}

% Python for inline
\newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}


%%%%%%%%%%%%%%




\begin{lstlisting}[language=Python, caption={Definition of \textbf{Heater} class}, label={lst:heater}]
import Pycatshoo as Pyc
class Heater(Pyc.CComponent):
...
 # heater states
    self.a1 = self.addAutomaton("Function") #Functioning
    self.stateOK  = self.addState("Function", "OK" , 1)
    self.stateNOK = self.addState("Function", "NOK", 0)
    self.setInitState("OK")
    
    self.a2 = self.addAutomaton("Power") #Control logic
    self.stateON  = self.addState("Power", "ON" , 1)
    self.stateOFF = self.addState("Power", "OFF", 0)
    self.setInitState("ON")
...
#heater transitions
    trans = self.stateOK.addTransition("OK_to_NOK")
    trans.setDistLaw(Pyc.IDistLaw.newLaw(self, Pyc.TLawType.expo, self.po_lambda))
...
    trans = self.stateOFF.addTransition("OFF_to_ON")
    trans.setDistLaw(Pyc.IDistLaw.newLaw(self, Pyc.TLawType.inst, 1))
    trans.setCondition("ONCondition",
    lambda: self.stateOK.isActive() and (self.getTemperature() <= self.po_minTemperature.dValue()), False)
...    
# Message boxes
    self.addMessageBox("mb_Room")
    self.addMessageBoxExport("mb_Room", self.stateON, "heaterON")
    self.addMessageBoxExport("mb_Room",self.po_power,"heatingPower)
    self.addMessageBoxImport("mb_Room",self.pi_roomTemperature,"temperature")
...
def stopCondition(self):
...
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Definition of \textbf{Room} class}, label={lst:room}]
import Pycatshoo as Pyc
class Room(Pyc.CComponent):
...
 # Message boxes
    self.addMessageBox("mb_Heater")
    self.addMessageBoxExport("mb_Heater", self.po_current_temperature, "temperature")
    self.addMessageBoxImport("mb_Heater", self.pi_heaterIsOn         , "heaterON")
...
# Creating PDMP Controller for the System 

    self.PDMP_temp = "pdmpTemperature"
    self.system().addPDMPManager(self.PDMP_temp)
    self.addPDMPEquationMethod(self.PDMP_temp, "pdmpMethod", None, 0)
    self.addPDMPODEVariable(self.PDMP_temp, self.po_current_temperature)
    self.addStartMethod("start", self.start)
...
    def pdmpMethod(self):
...
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Definition of \textbf{Room} class}, label={lst:hr}]
class HeatedRoomSystem(Pyc.CSystem):
    # Instantiation of heater and room
    self.heater = Heater("Heater")
    self.room   = Room("Room")

    # connecting heater and room via message boxes:
    self.connect("Heater", "mb_Room", "Room", "mb_Heater")
\end{lstlisting}

\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{LOC_ana}
  \caption{1a}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{CC_ana}
  \caption{1b}
  \label{fig:sfig2}
\end{subfigure}
\caption{plots of....}
\label{fig:fig}
\end{figure}

\begin{figure}   % the [b] specifies bottom of the page
\centering          % this centers everything inside the figure environment
\includegraphics[width=0.75\textwidth]{LOC_ana}
\caption{LOC analysis}
\label{fig:loc}
\end{figure}
\begin{figure}   % the [b] specifies bottom of the page
\centering          % this centers everything inside the figure environment
\includegraphics[width=0.75\textwidth]{CC_ana}
\caption{CC analysis}
\label{fig:cc}
\end{figure}

\begin{table}[]
\centering
\caption{Adaptive Maintainance of the Heated Room model}
\label{cases}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Case}: & \textbf{Modification type:} \\ \hline
\begin{tabular}[c]{@{ }l@{ }}\textbf{Case 0/0a:} \\A system with 1 heater and 1 room  \end{tabular} & Simplified model\\ \hline
\begin{tabular}[c]{@{ }l@{ }}\textbf{Case 1/1a: } \\ A system with 4 independent heaters \end{tabular} & \begin{tabular}[c]{@{ }l@{ }}\textbf{System level modifications:} \\ Scalability \end{tabular} \\ \hline
\begin{tabular}[c]{@{ }l@{ }}\textbf{Case 2/2a :} \\ A system with 4 heaters with passive \\ reservation (1 main and 3 backups) \end{tabular} & \begin{tabular}[c]{@{ }l@{ }}\textbf{Component level modifications:} \\ Modified control logic for heaters; \\ Dependencies between heaters\end{tabular} \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{Metrics for Maintainabiity Assessment of DPRA / PyCATSHOO models}
\label{metrics}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}\textbf{Metrics:}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Tool support:}} \\ \hline
\textbf{Size metrics:  LOC (lines of code)} & cloc, radon \\ \hline
\textbf{Complexity: Cyclomatic Complexity (CC)} & radon \\ \hline
\multicolumn{2}{|c|}{\textbf{Lexical measures:}} \\ \hline
Halstead (length, vocabulary, volume, effort, bugs, difficulty) & radon \\ \hline
\multicolumn{2}{|c|}{\textbf{Compound measures:}} \\ \hline
Maintainability Index (MI) & radon \\ \hline
\multicolumn{2}{|c|}{\textbf{OO-specific measures:}} \\ \hline
Chidamber \& Kemerer (WMC, DIT, NOC, CBO, RFC, LCOM) & -- \\ \hline
\multicolumn{2}{|c|}{\textbf{Structural complexity:}} \\ \hline
NC, NAgg, NGen, NGenH, MaxDIT … & -- \\ \hline
\end{tabular}
\end{table}
